Spectroscopic diagnostics of high-temperature plasma in stellar corona using Fe XXIV--XXVI K-shell lines with XRISM

The RS CVn type binary star GT Mus was observed during its quiescence using the Resolve X-ray microcalorimeter spectrometer onboard XRISM. The main and satellite lines of the Fe XXIV--XXVI K-shell transitions were resolved for the first time from stellar sources. We conducted line ratio analysis to investigate any deviations from collisional onization equilibrium (CIE) and Maxwell electron energy distribution with a single-temperature. By using five combinations of direct excitation lines and dielectronic recombination satellite lines in three line complexes (Fe He$\alpha$, Ly$\alpha$, and He$\beta$), we found that the plasma is well characterized by two-temperature thermal plasmas with temperatures of 1.7 and 4.3 keV, which is consistent with a thermal broadening of Fe XXV and the broadband fitting results in the 1.7--10 keV band. Other forms of deviation from a single-temperature plasma, such as different ionization and electron temperatures or the $\kappa$ distribution for the electron energy distributions, are not favored, which is reasonable for stellar coronae at quiescence. This study demonstrates the utility of the Fe K-shell line ratio diagnostics to probe plasma conditions using X-ray microcalorimeters.

==> Makefile <==
# Time-stamp: <Wed Feb 14 09:15:10 JST 2024>

############################################################
# ソースファイル
############################################################
# ソースファイル（必須）
SRC	= ms.tex


############################################################
# 書式の設定（必須）
############################################################
ENGINE  = pdf   # "pdf" for pdflatex, "lua" for lualatex, "up" for uplatex.
BIBTEX  = yes    # "yes" for BIBER, "no" for BIBTEX.
OVERLEAF= yes   # "yes" for overleaf, "no" for else.
A4      = yes   # "yes" for A4, "no" for US Letter.
LNDSCP  = no    # "yes" for landscape, "no" for portrait.

############################################################
# コンパイル時の処理（optional）
############################################################
COMPRESSFILES 	= # Compress に含むファイル（追加分のみ）

# コンパイル前の処理
compile_prehook_usr: $(BIBS)

# #	$(BIBTOOL) -o $(subst .tex,.bib,$(SRC)) -i $(BIBFILES) -s -d

# 	@for i in $(FIGURES) ; do \
# 	num=`echo $${i} | cut -c 2-3` ; \
# 	[ -f $${i} ] || $(LN) ../Figures/$${num}/$${i} . ; \
# 	$(PDFSPLIT) $${i} ; \
# 	done

# 	@for i in $(TABLES) ; do \
# 	num=`echo $${i} | cut -c 2-3` ; \
# 	[ -f $${i} ] || $(LN) ../Tables/$${num}/$${i} . ; \
# 	$(PDFSPLIT) $${i} ; \
# 	done

	-@$(EBB) $(FIGURES) $(TABLES)

# コンパイル後の処理
compile_posthook_usr:

############################################################
# コマンド設定（変更不要）
############################################################
MAKEFILEDIR	= ${HOME}/Work/.templates/LaTeX
include		${MAKEFILEDIR}/Makefile

